SRoll3: A neural network approach to reduce large-scale systematic effects in the Planck High Frequency Instrument maps

In the present work, we propose a neural network based data inversion approach to reduce structured contamination sources, with a particular focus on the mapmaking for Planck High Frequency Instrument (Planck-HFI) data and the removal of large-scale systematic effects within the produced sky maps. The removal of contamination sources is rendered possible by the structured nature of these sources, which is characterized by local spatiotemporal interactions producing couplings between different spatiotemporal scales. We focus on exploring neural networks as a means of exploiting these couplings to learn optimal low-dimensional representations, optimized with respect to the contamination source removal and mapmaking objectives, to achieve robust and effective data inversion. We develop multiple variants of the proposed approach, and consider the inclusion of physics informed constraints and transfer learning techniques. Additionally, we focus on exploiting data augmentation techniques to integrate expert knowledge into an otherwise unsupervised network training approach. We validate the proposed method on Planck-HFI 545 GHz Far Side Lobe simulation data, considering ideal and non-ideal cases involving partial, gap-filled and inconsistent datasets, and demonstrate the potential of the neural network based dimensionality reduction to accurately model and remove large-scale systematic effects. We also present an application to real Planck-HFI 857 GHz data, which illustrates the relevance of the proposed method to accurately model and capture structured contamination sources, with reported gains of up to one order of magnitude in terms of contamination removal performance. Importantly, the methods developed in this work are to be integrated in a new version of the SRoll algorithm (SRoll3), and we describe here SRoll3 857 GHz detector maps that will be released to the community.

==> shortcuts.tex <==
\def\result#1{\vspace{5pt}\noindent\textbf{#1}---}
\def\fnllocal{f_\textrm {NL}^\textrm{local}}
\def\LCDM{$\Lambda$CDM}
\def\NHUNIT{\ifmmode {\rm \,cm^{-2}} \else $\rm \,cm^{-2}$ \fi} % NH units
\def\clee{$C_\ell^{EE}$}
\def\clbb{$C_\ell^{BB}$}
\def\wmap{\WMAP}
\def\aap{{A\&A}}
\def\apj{{ApJ}}
\def\mnras{{MNRAS}}
\def\apjs{{ApJ Supp.}}
\def\muKcmb{\ifmmode \,\mu$K$_{\rm CMB}$\else \,$\mu$K$_{\rm CMB}$\fi}
%
\newcommand{\NH}{N_{\rm H}} % NH
%
\newcommand{\planck}{\Planck}
\newcommand{\WMAP}{WMAP}
\newcommand{\WP}{WP}
\newcommand{\highL}{highL}
\newcommand{\lensing}{lensing}
\newcommand{\planckonly}{\planck}
\newcommand{\plancklensing}{\planck+\lensing}
\newcommand{\HighL}{\highL}

\newcommand{\As}{A_{\rm s}}
\newcommand{\At}{A_{\rm t}}
\newcommand{\nt}{n_{\rm t}}
\newcommand{\ns}{n_{\rm s}}
\newcommand{\lcdm}{$\Lambda$CDM}
\newcommand{\rpivot}{r_{0.05}}
\newcommand{\rzerotwo}{r_{0.002}}
\newcommand{\Alens}{A_{\rm L}}
\newcommand{\Aphiphi}{A_{\rm L}^{\phi\phi}}
\newcommand{\omegak}{\Omega_K}
\newcommand{\omegal}{\Omega_\Lambda}
\newcommand{\OmegaM}{\ifmmode\Omega_{\rm M}\else $\Omega_{\rm M}$\fi}

\newcommand{\nrun}{d \ns / d\ln k}
\newcommand{\zre}{z_{\text{re}}}
\newcommand{\yhe}{Y_{\text{P}}}
\newcommand{\zeq}{z_{\text{eq}}}
\newcommand{\nnu}{N_{\rm eff}}
\newcommand{\neff}{N_{\rm eff}}
\newcommand{\mnu}{\sum m_\nu}
\newcommand{\sumnu}{\sum m_\nu}
\newcommand{\mnusterile}{m_{\nu,\, \mathrm{sterile}}^{\mathrm{eff}}}

\newcommand{\zdrag}{z_{\rm drag}}
\newcommand{\rdrag}{r_{\rm drag}}
\newcommand{\zstar}{z_{\ast}}
\newcommand{\rstar}{r_{\ast}}
\newcommand{\rs}{r_{\rm s}}
\newcommand{\thetastar}{\theta_{\ast}}
\newcommand{\DAstar}{D_{\rm A}}

\newcommand{\Ailensbestfit}{A_i^{\mbox{\scriptsize{theory}}}}
\newcommand{\Alensbestfit}{A^{\mbox{\scriptsize{theory}}}}

\newcommand{\efhcite}[1]{{\bf #1}}

\newcommand{\typeone}{{\sc{Type~1}}}
\newcommand{\typetwo}{{\sc{Type~2}}}
\newcommand{\typethree}{{\sc{Type~3}}}
\newcommand{\joz}{$J$=1$\rightarrow$0}
\newcommand{\jto}{$J$=2$\rightarrow$1}
\newcommand{\jtt}{$J$=3$\rightarrow$2}
\newcommand{\cooz}{CO(1$\rightarrow$0)}
\newcommand{\coto}{CO(2$\rightarrow$1)}
\newcommand{\cott}{CO(3$\rightarrow$2)}

\renewcommand{\topfraction}{1.0}  % max fraction of floats at top
    \renewcommand{\bottomfraction}{1.0} % max fraction of floats at bottom
    %   Parameters for TEXT pages (not float pages):
    \setcounter{topnumber}{2}
    \setcounter{bottomnumber}{2}
    \setcounter{totalnumber}{4}     % 2 may work better
    \setcounter{dbltopnumber}{2}    % for 2-column pages
    \renewcommand{\dbltopfraction}{0.9} % fit big float above 2-col. text
    \renewcommand{\textfraction}{0.00}  % allow minimal text w. figs
    %   Parameters for FLOAT pages (not text pages):
    \renewcommand{\floatpagefraction}{0.9}  % require fuller float pages
  % N.B.: floatpagefraction MUST be less than topfraction !!
    \renewcommand{\dblfloatpagefraction}{0.9} % require fuller float pages

\newcommand{\FRB}[1]{\textcolor{red}{$\triangleleft$ FRB: #1 $\triangleright$}}
% \newcommand{\PN}[1]{\textcolor{blue}{$\triangleleft$ PN: #1 $\triangleright$}}
% \newcommand{\EFH}[1]{\textcolor{cyan}{\textbf{$\triangleleft$ EFH: #1 $\triangleright$}}}
% \newcommand{\SG}[1]{\textcolor{magenta}{\textbf{$\triangleleft$ SG: #1 $\triangleright$}}}
% \newcommand{\HKE}[1]{\textcolor{green}{\textbf{$\triangleleft$ HKE: #1 $\triangleright$}}}
%
\def\WMAP{{WMAP}}
\def\COBE{{COBE}}

\newcommand{\onesig}[1]{(68\%, \text{#1})}
\newcommand{\twosig}[1]{(95\%, \text{#1})}
\newcommand{\twoonesig}[3]{
\begin{equation}
\left.
 \begin{aligned}
#1 \\ #2
 \end{aligned}
\ \right\} \ \ \mbox{\text{#3}}
\end{equation}
}
\newcommand{\twotwosig}[3]{
\begin{equation}
\left.
 \begin{aligned}
#1 \\ #2
 \end{aligned}
\ \right\} \ \ \mbox{95\%, \text{#3}}
\end{equation}
}


\newcommand{\ncib}{\gamma^{\rm CIB}}
\newcommand{\camspec}{{\tt CamSpec}}
\newcommand{\plik}{{\tt Plik}}
\newcommand{\pliklite}{\texttt{Plik\_lite}}
\newcommand{\plikclean}{\textcolor{red}{TEMPORARY \texttt{Plik\_clean}}}

\newcommand{\commander}{{\tt Commander}}
\newcommand{\mspec}{{\tt MSPEC}}
\newcommand{\smica}{{\tt SMICA}}

\newcommand{\CFHTLENS}{CFHTLenS}
\newcommand{\meanchisquare}{\overline{\chi^2}}



\newcommand{\thetaMC}{\theta_{\rm MC}}
\newcommand{\ypbbn}{Y_{\text{P}}^{\rm BBN}}
\newcommand{\meffsterile}{\mnusterile}
\newcommand{\Tactive}{T_{\mathrm{a}}}
\newcommand{\Tsterile}{T_{\mathrm{s}}}
\newcommand{\msthermal}{m_{\rm sterile}^{\rm thermal}}
\newcommand{\msDW}{m_{\rm sterile}^{\rm DW}}

\newcommand{\keq}{k_{\rm eq}}
\newcommand{\DVBAO}{D_{\rm V}}
\newcommand{\DA}{D_{\rm A}}




% Alter some LaTeX defaults for better treatment of figures:
% See p.105 of "TeX Unbound" for suggested values.
% See pp. 199-200 of Lamport's "LaTeX" book for details.
%   General parameters, for ALL pages:
\renewcommand{\topfraction}{0.9}    % max fraction of floats at top
\renewcommand{\bottomfraction}{0.8} % max fraction of floats at bottom
    %   Parameters for TEXT pages (not float pages):
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}     % 2 may work better
\setcounter{dbltopnumber}{2}    % for 2-column pages
\renewcommand{\dbltopfraction}{0.9} % fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}  % allow minimal text w. figs
%   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.7}  % require fuller float pages
    % N.B.: floatpagefraction MUST be less than topfraction !!
\renewcommand{\dblfloatpagefraction}{0.7}   % require fuller float pages

% remember to use [htp] or [htpb] for placement


\newcommand{\fixme}[1]{{\color{Red}{ FIXME: #1}}}
\newcommand{\quietfixme}[1]{{\color{Red} #1}}
\newcommand{\notate}[1]{{\color{olive} NOTE: #1}}

\newcommand{\fnl}{f_{\rm{NL}}}
\newcommand{\fnlloc}{f^{\rm local}_{\rm NL}}
\newcommand{\fnleqi}{f^{\rm equil}_{\rm NL}}
\newcommand{\taunl}{\tau_{\rm{NL}}}
\newcommand{\gnl}{g_{\rm{NL}}}
\newcommand{\htaunl}{\hat{\tau}_{\rm NL}}

\providecommand{\Planck}{\textit{Planck}}
\providecommand{\planck}{\Planck}
\newcommand{\covinvT}{\bar{\Theta}}
\newcommand{\Ltemp}{\tilde{T}}
\newcommand{\lensedC}{\tilde{C}}
\newcommand{\Lmin}{{L_{\rm min}}}

%\providecommand{\lea}{\lesssim}
%\providecommand{\gea}{\gtrsim}
\providecommand{\lea}{\la}
\providecommand{\gea}{\ga}


\providecommand{\alt}{\lea}
\providecommand{\agt}{\gea}
\providecommand{\text}[1]{\rm{#1}}



\newcommand{\Msun}{M_\odot}
\newcommand{\tot}{{\text{tot}}}
\newcommand{\Mpc}{\text{Mpc}}
\newcommand{\half}{{\textstyle \frac{1}{2}}}
\newcommand{\third}{{\textstyle \frac{1}{3}}}
\newcommand{\numfrac}[2]{{\textstyle \frac{#1}{#2}}}
\renewcommand{\d}{\text{d}}
\newcommand{\grad}{\nabla}
\newcommand{\km}{\rm{\,km\,}}

\newcommand{\Hunit}{~\text{km}~\text{s}^{-1} \Mpc^{-1}}
\newcommand{\Gyr}{{\rm Gyr}}
\providecommand{\muK}{\mu\rm{K}}
\newcommand{\muKarcmin}{\,\muK\,\arcmin}
\newcommand{\muKsq}{(\mu\rm{K})^2}
\newcommand{\lmax}{l_{\text{max}}}
\newcommand{\lmin}{l_{\text{min}}}

\newcommand{\mpl}{m_{\text{Pl}}}
\newcommand{\eV}{\,\text{eV}}
\newcommand{\MeV}{\,\text{MeV}}
\newcommand{\GeV}{\,\text{GeV}}


\providecommand{\Omk}{\Omega_K}
\providecommand{\Oml}{\Omega_{\Lambda}}
\providecommand{\Omtot}{\Omega_{\mathrm{tot}}}
\providecommand{\Omb}{\Omega_{\mathrm{b}}}
\providecommand{\Omc}{\Omega_{\mathrm{c}}}
\providecommand{\Omm}{\Omega_{\mathrm{m}}}
\providecommand{\omb}{\omega_{\mathrm{b}}}
\providecommand{\omc}{\omega_{\mathrm{c}}}
\providecommand{\omm}{\omega_{\mathrm{m}}}
\providecommand{\Omdm}{\Omega_{\mathrm{DM}}}
\providecommand{\Omnu}{\Omega_{\nu}}

\providecommand{\CAMB}{{\tt camb}}
\providecommand{\COSMOMC}{{\tt CosmoMC}}
\providecommand{\CMBFAST}{{\tt cmbfast}}
\providecommand{\COSMICS}{{\tt Cosmics}}
\providecommand{\CLASS}{{\tt class}}
\providecommand{\CMBEASY}{{\tt cmbeasy}}
\providecommand{\LCDM}{{$\rm{\Lambda CDM}$}}
\providecommand{\COSMOREC}{{\tt CosmoRec}}
\providecommand{\HYREC}{{\tt HyRec}}
\providecommand{\RECFAST}{{\tt recfast}}
\providecommand{\HALOFIT}{{\tt halofit}}
\providecommand{\AlterBBN}{{\tt AlterBBN}}
\providecommand{\MontePython}{{\tt Monte Python}}
\providecommand{\HEALpix}{{\tt HEALpix}}


\newcommand{\begm}{\begin{pmatrix}}
\newcommand{\enm}{\end{pmatrix}}
\newcommand{\threej}[6]{{\begm #1 & #2 & #3 \\ #4 & #5 & #6 \enm}}
\newcommand{\threejz}[3]{{\begm #1 & #2 & #3 \\ 0 & 0 & 0 \enm}}





\newcommand{\valpha}{{\boldsymbol{pha}}}
\newcommand{\vgrad}{{\boldsymbol{\nabla}}}
\newcommand{\vpsi}{\mathbf{\psi}}
\newcommand{\vTheta}{\mathbf{\Theta}}
\newcommand{\vdelta}{\boldsymbol{\delta}}


%%%%% statistics %%%%%%%%%%%%

%Variance
\providecommand{\var}{\text{var}}
%covariance
\providecommand{\cov}{\text{cov}}

\providecommand{\Tr}{\text{Tr}}
%likelihood

%integration
\newcommand{\ud}{{\rm d}}


%%%%%%% Matrices %%%%%%%%%%
\newcommand{\mA}{\bm{A}}
\newcommand{\mB}{\bm{B}}
\newcommand{\mC}{\bm{C}}
\newcommand{\mD}{\bm{D}}
\newcommand{\mE}{\bm{E}}
\newcommand{\mF}{\bm{F}}
\newcommand{\mG}{\bm{G}}
\newcommand{\mH}{\bm{H}}
\newcommand{\mI}{\bm{I}}
\newcommand{\mJ}{\bm{J}}
\newcommand{\mK}{\bm{K}}
\newcommand{\mL}{\bm{L}}
\newcommand{\mM}{\bm{M}}
\newcommand{\mN}{\bm{N}}
\newcommand{\mO}{\bm{O}}
\newcommand{\mP}{\bm{P}}
\newcommand{\mQ}{\bm{Q}}
\newcommand{\mR}{\bm{R}}
\newcommand{\mS}{\bm{S}}
\newcommand{\mT}{\bm{T}}
\newcommand{\mU}{\bm{U}}
\newcommand{\mV}{\bm{V}}
\newcommand{\mW}{\bm{W}}
\newcommand{\mX}{\bm{X}}
\newcommand{\mY}{\bm{Y}}
\newcommand{\mZ}{\bm{Z}}

\newcommand{\mLambda}{\bm{\Lambda}}
\newcommand{\mzero}{\bm{0}}

%%%%%%%% Vectors %%%%%%%%%%

\newcommand{\boldvec}[1]{{\mbox{\boldmath{$#1$}}}}

\newcommand{\vA}{\boldvec{A}}
\newcommand{\vB}{\boldvec{B}}
\newcommand{\vC}{\boldvec{C}}
\newcommand{\vD}{\boldvec{D}}
\newcommand{\vE}{\boldvec{E}}
\newcommand{\vF}{\boldvec{F}}
\newcommand{\vG}{\boldvec{G}}
\newcommand{\vH}{\boldvec{H}}
\newcommand{\vI}{\boldvec{I}}
\newcommand{\vJ}{\boldvec{J}}
\newcommand{\vK}{\boldvec{K}}
\newcommand{\vL}{\boldvec{L}}
\newcommand{\vM}{\boldvec{M}}
\newcommand{\vN}{\boldvec{N}}
\newcommand{\vO}{\boldvec{O}}
\newcommand{\vP}{\boldvec{P}}
\newcommand{\vQ}{\boldvec{Q}}
\newcommand{\vR}{\boldvec{R}}
\newcommand{\vS}{\boldvec{S}}
\newcommand{\vT}{\boldvec{T}}
\newcommand{\vU}{\boldvec{U}}
\newcommand{\vV}{\boldvec{V}}
\newcommand{\vW}{\boldvec{W}}
\newcommand{\vX}{\boldvec{X}}
\newcommand{\vY}{\boldvec{Y}}
\newcommand{\vZ}{\boldvec{Z}}

\newcommand{\va}{\boldvec{a}}
\newcommand{\vb}{\boldvec{b}}
\newcommand{\vc}{\boldvec{c}}
\newcommand{\vd}{\boldvec{d}}
\newcommand{\ve}{\boldvec{e}}
\newcommand{\vf}{\boldvec{f}}
\newcommand{\vg}{\boldvec{g}}
\newcommand{\vh}{\boldvec{h}}
\newcommand{\vi}{\boldvec{i}}
\newcommand{\vj}{\boldvec{j}}
\newcommand{\vk}{\boldvec{k}}
\newcommand{\vl}{\boldvec{l}}
\newcommand{\vm}{\boldvec{m}}
\newcommand{\vn}{\boldvec{n}}
\newcommand{\vo}{\boldvec{o}}
\newcommand{\vp}{\boldvec{p}}
\newcommand{\vq}{\boldvec{q}}
%\newcommand{\vr}{\boldvec{r}}
\newcommand{\vs}{\boldvec{s}}
\newcommand{\vt}{\boldvec{t}}
\newcommand{\vu}{\boldvec{u}}
\newcommand{\vv}{\boldvec{v}}
\newcommand{\vw}{\boldvec{w}}
\newcommand{\vx}{\boldvec{x}}
\newcommand{\vy}{\boldvec{y}}
\newcommand{\vz}{\boldvec{z}}

\newcommand{\cla}{\mathcal{A}}
\newcommand{\clb}{\mathcal{B}}
\newcommand{\clc}{\mathcal{C}}
\newcommand{\cld}{\mathcal{D}}
\newcommand{\cle}{\mathcal{E}}
\newcommand{\clf}{\mathcal{F}}
\newcommand{\clg}{\mathcal{G}}
\newcommand{\clh}{\mathcal{H}}
\newcommand{\cli}{\mathcal{I}}
\newcommand{\clj}{\mathcal{J}}
\newcommand{\clk}{\mathcal{K}}
\newcommand{\cll}{\mathcal{L}}
\newcommand{\clm}{\mathcal{M}}
\newcommand{\cln}{\mathcal{N}}
\newcommand{\clo}{\mathcal{O}}
\newcommand{\clp}{\mathcal{P}}
\newcommand{\clq}{\mathcal{Q}}
\newcommand{\clr}{\mathcal{R}}
\newcommand{\cls}{\mathcal{S}}
\newcommand{\clt}{\mathcal{T}}
\newcommand{\clu}{\mathcal{U}}
\newcommand{\clv}{\mathcal{V}}
\newcommand{\clw}{\mathcal{W}}
\newcommand{\clx}{\mathcal{X}}
\newcommand{\cly}{\mathcal{Y}}
\newcommand{\clz}{\mathcal{Z}}



\newcommand{\vnhat}{\hat{\vn}}
\newcommand{\vrhat}{\hat{\vr}}
\newcommand{\vkhat}{\hat{\vk}}

\def\pmb#1{\setbox0=\hbox{#1}%
    \kern-.025em\copy0\kern-\wd0
    \kern.05em\copy0\kern-\wd0
    \kern-.025em\raise.0433em\box0}
%\def\ltsima{$\; \buildrel < \over \sim \;$}
%\def\gtsima{$\; \buildrel > \over \sim \;$}
%\def\simlt{\lower.5ex\hbox{\ltsima}}
%\def\simgt{\lower.5ex\hbox{\gtsima}}

\providecommand{\ltsima}{\lea}
\providecommand{\gtsima}{\gea}
\providecommand{\simlt}{\lea}
\providecommand{\simgt}{\gea}

\def\muk{$(\mu{\rm K})^2$ }
\def\etal{{et al.}}
\def\etals{{et al. }}
\def\p2Y{\;_2Y}
\def\m2Y{\;_{-2}Y}
%\newcounter{parentequation}\setcounter{parentequation}{0}
\def\beglet{
  \addtocounter{equation}{1}%
  \setcounter{parentequation}{\value{equation}}%
  \setcounter{equation}{0}%
  \def\theequation{\arabic{parentequation}\alph{equation}}%
  \ignorespaces
}
\def\endlet{
  \setcounter{equation}{\value{parentequation}}%
  \def\theequation{\arabic{equation}}%
}
%amsmath already has subequation support
\providecommand{\beglet}{\begin{subequations}}
\providecommand{\endlet}{\end{subequations}}


\def\ExpSup{\citep{planck2013-p28}}

\newcommand{\elec}{{\rm e}}
\newcommand{\neutron}{{\rm n}}

\newcommand{\mksym}[1]{\ifmmode {\rm #1}\else #1\fi}

\newcommand{\plikTT}{\texttt{Plik}\rm TT}
\newcommand{\plikEE}{\texttt{Plik}\rm EE}
\newcommand{\plikTE}{\texttt{Plik}\rm TE}

\newcommand{\ext}{\mksym{{\rm ext}}}
\newcommand{\TT}{\mksym{{\rm TT}}}
\newcommand{\EE}{\mksym{{\rm EE}}}
\newcommand{\BB}{\mksym{{\rm BB}}}
\newcommand{\TE}{\mksym{{\rm TE}}}
\newcommand{\ET}{\mksym{{\rm ET}}}
\newcommand{\TB}{\mksym{{\rm TB}}}
\newcommand{\EB}{\mksym{{\rm EB}}}


\newcommand{\TTTEEE}{\mksym{{\rm TT{,}TE{,}EE}}}
\newcommand{\planckTTonly}{{\rm PlanckTT}}
\newcommand{\planckTEonly}{{\rm PlanckTE}}
\newcommand{\planckEEonly}{{\rm PlanckEE}}
\newcommand{\lowTEB}{\mksym{{\rm lowTEB}}}
\newcommand{\lowEB}{\mksym{{\rm lowP}}}
\newcommand{\lowTP}{\mksym{{\rm lowT{,}P}}}
\newcommand{\planckTT}{{\rm PlanckTT{+}\lowEB}}
\newcommand{\planckall}{{\rm PlanckTT,TE,EE{+}\lowEB}}
\newcommand{\shortTT}{{\plikTT{+}\lowTEB}}
\newcommand{\shortTE}{{\plikTE{+}\lowTEB}}
\newcommand{\shortEE}{{\plikEE{+}\lowTEB}}
\newcommand{\shortall}{{\plikTTTEEE{+}\lowTEB}}
\newcommand{\planckTTTEEE}{{\rm PlanckTT,TE,EE}}

\newcommand{\lnAs}{\ln(10^{10} A_{\rm s})}







% Alter some LaTeX defaults for better treatment of figures:
% See p.105 of "TeX Unbound" for suggested values.
% See pp. 199-200 of Lamport's "LaTeX" book for details.
%   General parameters, for ALL pages:
\renewcommand{\topfraction}{0.9}    % max fraction of floats at top
\renewcommand{\bottomfraction}{0.8} % max fraction of floats at bottom
    %   Parameters for TEXT pages (not float pages):
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}     % 2 may work better
\setcounter{dbltopnumber}{2}    % for 2-column pages
\renewcommand{\dbltopfraction}{0.9} % fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}  % allow minimal text w. figs
%   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.7}  % require fuller float pages
    % N.B.: floatpagefraction MUST be less than topfraction !!
\renewcommand{\dblfloatpagefraction}{0.7}   % require fuller float pages

% remember to use [htp] or [htpb] for placement




%\providecommand{\Planck}{\textit{Planck}}
%\providecommand{\planck}{\Planck}

\providecommand{\lea}{\lesssim}
\providecommand{\gea}{\gtrsim}


\providecommand{\alt}{\lea}
\providecommand{\agt}{\gea}
\providecommand{\text}[1]{\rm{#1}}



\renewcommand{\d}{\text{d}}

\providecommand{\muK}{\mu\rm{K}}
  


\providecommand{\Omk}{\Omega_K}
\providecommand{\Oml}{\Omega_{\Lambda}}
\providecommand{\Omtot}{\Omega_{\mathrm{tot}}}
\providecommand{\Omb}{\Omega_{\mathrm{b}}}
\providecommand{\Omc}{\Omega_{\mathrm{c}}}
\providecommand{\Omm}{\Omega_{\mathrm{m}}}
\providecommand{\omb}{\omega_{\mathrm{b}}}
\providecommand{\omc}{\omega_{\mathrm{c}}}
\providecommand{\omm}{\omega_{\mathrm{m}}}
\providecommand{\Omdm}{\Omega_{\mathrm{DM}}}
\providecommand{\Omnu}{\Omega_{\nu}}


\newcommand{\Omch}{\Omega_{\mathrm{c}}h^2}
\newcommand{\Ombh}{\Omega_{\mathrm{b}}h^2}
\newcommand{\clamp}{\As \exp{-2\tau}}


%%%% AHJ: I think these should all be typewriter font (\textt)
\providecommand{\healpix}{\texttt{HEALPix}}
 
\providecommand{\CAMB}{\texttt{CAMB}}
\providecommand{\COSMOMC}{\texttt{CosmoMC}}
\providecommand{\CMBFAST}{\texttt{CMBFAST}}
\providecommand{\COSMICS}{\texttt{COSMICS}}
\providecommand{\CLASS}{\texttt{CLASS}}
\providecommand{\CMBEASY}{\texttt{CMBEasy}}
\providecommand{\COSMOREC}{\texttt{CosmoRec}}
\providecommand{\HYREC}{\texttt{HyRec}}
\providecommand{\RECFAST}{\texttt{RecFast}}
\providecommand{\HALOFIT}{\texttt{HaloFit}}
\providecommand{\PICO}{\texttt{PICO}}

% \providecommand{\CAMB}{\textsc{camb}}
% \providecommand{\COSMOMC}{\textsc{CosmoMC}}
% \providecommand{\CMBFAST}{\textsc{cmbfast}}
% \providecommand{\COSMICS}{\textsc{Cosmics}}
% \providecommand{\CLASS}{\textsc{class}}
% \providecommand{\CMBEASY}{\textsc{cmbeasy}}
% \providecommand{\COSMOREC}{\textsc{CosmoRec}}
% \providecommand{\HYREC}{\textsc{HyRec}}
% \providecommand{\RECFAST}{\textsc{recfast}}
% \providecommand{\HALOFIT}{\textsc{halofit}}
% \providecommand{\PICO}{\textsc{pico}}

\providecommand{\LCDM}{{$\rm{\Lambda CDM}$}}




\newcommand\ba{\begin{eqnarray}}
\newcommand\ea{\end{eqnarray}}
\newcommand\bea{\begin{eqnarray}}
\newcommand\eea{\end{eqnarray}}

\newcommand\be{\begin{equation}}
\newcommand\ee{\end{equation}}






%%%%% statistics %%%%%%%%%%%%

%Variance
\providecommand{\var}{\text{var}}
%covariance
\providecommand{\cov}{\text{cov}}

\providecommand{\Tr}{\text{Tr}}
%likelihood

%integration


%%%%%%% Matrices %%%%%%%%%%


%%%%%%%% Vectors %%%%%%%%%%







%\def\pmb#1{\setbox0=\hbox{#1}%
%    \kern-.025em\copy0\kern-\wd0
%    \kern.05em\copy0\kern-\wd0
%    \kern-.025em\raise.0433em\box0}
%\def\ltsima{$\; \buildrel < \over \sim \;$}
%\def\gtsima{$\; \buildrel > \over \sim \;$}
%\def\simlt{\lower.5ex\hbox{\ltsima}}
%\def\simgt{\lower.5ex\hbox{\gtsima}}
%\def\muk{$(\mu{\rm K})^2$ }
%\def\etal{{\it et al.}}
%\def\etals{{\it et al. }}
%\def\p2Y{\;_2Y}
%\def\m2Y{\;_{-2}Y}
%\newcounter{parentequation}\setcounter{parentequation}{0}
%\def\beglet{
%  \addtocounter{equation}{1}%
%  \setcounter{parentequation}{\value{equation}}%
%  \setcounter{equation}{0}%
%  \def\theequation{\arabic{parentequation}\alph{equation}}%
%  \ignorespaces
%}
%\def\endlet{
%  \setcounter{equation}{\value{parentequation}}%
%  \def\theequation{\arabic{equation}}%
%}

\def\PaperI{\citep{planck2013-p08}}

\def\ExpSup{\citep{planck2013-p28}}

\newcommand{\dagme}[1]{\textcolor{red}{$\dagger$ #1 $\dagger$}}
\newcommand{\kb}[1]{\textcolor{pink}{$\dagger$ #1 $\dagger$}}
\newcommand{\ghz}{GHz}
\newcommand{\SG}[1]{\textcolor{teal}{$\dagger$ #1 $\dagger$}}
